Distilled GPT for Source Code Summarization

A code summary is a brief natural language description of source code. Summaries are usually only a single sentence long, and yet form the backbone of developer documentation. A short descriptions such as "changes all visible polygons to the color blue" can give a programmer a high-level idea of what code does without the effort of reading the code itself. Recently, products based on Large Language Models such as ChatGPT have demonstrated a strong ability to write these descriptions automatically. However, to use these tools, programmers must send their code to untrusted third parties for processing (e.g., via an API call). This loss of custody is not acceptable to many organizations. In this paper, we present an alternative: we train an open source model using sample output generated by GPT-3.5 in a process related to knowledge distillation. Our model is small enough (350m parameters) to be run on a single 16gb GPU, yet we show in our evaluation that it is large enough to mimic GPT-3.5 on this task.

==> background.tex <==
\section{Background and Related Work}
\label{sec:background}

This section discusses the two key areas of background and related work: code summarization and knowledge distillation.

\subsection{Source Code Summarization}

The term ``source code summarization'' was coined in 2010 by~\citet{haiduc2010use} to refer to the task of writing natural language descriptions of code.  Until 2017, most of research methods focused on IR-based and template-based methods. From 2017 to present, neural models for code summairzation becomes the most dominant research direction. Table~\ref{tab:screlated} shows the history and families of different methods. Although the most dominant research line is neural models, there are different families of neural models, which include better modeling of code itself and using more context. For example,~\citet{leclair2019neural, alon2019code2seq, alon2019code2vec} combined AST with source code and  \citet{allamanis2018learning} modeled AST as a graph for neural models.~\citet{haque2020improved} applied the attention mechanism to the file context.~\citet{bansal2021project} combined information different software projects.

More recently, large language models (LLM) such as OpenAI's ChatGPT have demonstrated the great capability on program comprehension. However, it is hard to avoid data leak problems when we use these models for research because the training data of these models is not publicly accessible. In this paper, we distill the knowledge from GPT-3.5 by training small models with public and controllable datasets and mimic GPT-3.5's capability for code summarization.

\begin{table*}[!b]
    \centering
	{\small
    
		\begin{tabular}{p{4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}}
        \centering
			& I     & N          & G          & T & C                \\
			\citet{mcburney2016automated}						& x &  	&   &   & x \\
			%\textcolor{white}{*}Zhang~\emph{et al.}~(2016)~\cite{zhang2016towards}					& x &  	&   &   & x \\
			%\textcolor{white}{*}Iyer~\emph{et al.}~(2016)~\cite{iyer2016summarizing}				&   & x &   &   &   \\
			\citet{rodeghero2017detecting}		& x &  	&   &   & x \\
			\citet{fowkes2017autofolding}			& x &  	&   &   &   \\
			%\textcolor{white}{*}Badihi~\emph{et al.}~(2017)~\cite{badihi2017crowdsummarizer}		& x &  	&   &   &   \\
			%\textcolor{white}{*}Loyola~\emph{et al.}~(2017)~\cite{loyola2017neural}					&   & x	&   &   &   \\
			%\textcolor{white}{*}Lu~\emph{et al.}~(2017)~\cite{lu2017learning}						&   & x	&   &   &   \\
			\citet{jiang2017automatically}			&   & x	&   &   &   \\
			%\textcolor{white}{*}Hu~\emph{et al.}~(2018)~\cite{hu2018summarizing}					&   & x	&   &   &   \\
			\citet{hu2018deep}							&   & x	& x &   &   \\
			\citet{allamanis2018learning}			&   & x	& x &   &   \\
			%\textcolor{white}{*}Wan~\emph{et al.}~(2018)~\cite{wan2018improving}					&   & x	&   &   &   \\
			%\textcolor{white}{*}Liang~\emph{et al.}~(2018)~\cite{liang2018automatic}				&   & x	&   &   &   \\
			\citet{alon2019code2seq, alon2019code2vec}	&   & x	& x &   &   \\
			\cite{gao2019neural}						&   & x	&   &   &   \\
			\citet{leclair2019neural}				&   & x	& x &   &   \\
			~\citet{nie2019framework}					&   & x	&   &   &   \\
			%\textcolor{white}{*}Haldar~\emph{et al.}~(2020)~\cite{haldar2020multi}					&   & x	&   &   &   \\
			%\textcolor{white}{*}Ahmad~\emph{et al.}~(2020)~\cite{ahmad2020transformer}				&   & x	&   & x &   \\
			\citet{haque2020improved}					&   & x	&   &   & x \\ 
			\citet{zugner2021languageagnostic}	&   & x	& x &   &   \\
			\citet{liu2021retrievalaugmented}			&   & x	& x &   &   \\
			\citet{bansal2021project}				&   &x       &    &   & x \\
			%\textcolor{white}{*}  (This Paper)											&   &x       &x  &   &x \\
		\end{tabular}
	}
	\vspace{0.2cm}
	\caption{Snapshot of the past five years in source code summarization.  Column $I$ stands for IR-based techniques.  $N$ means neural network-based.  $G$ means the code is modeled as a graph.  $T$ means Transformer designs.  $C$ means learning from context.}
	\label{tab:screlated}
\end{table*}

\subsection{Knowledge Distillation}

Knowledge Distillation refers to teaching a small machine learning model to behave like a larger one for a niche task~\citep{wang2021knowledge}.  Knowledge distillation is useful in scenarios where a large model may be capable of many tasks or even considered general purpose, such as ChatGPT or Copilot, but is too expensive or impractical to use for certain specific tasks.  A classic application is in image classification, where a powerful model capable of classifying many types may be used to teach a smaller model with some tradeoffs, such as lower accuracy or recognizing fewer categories~\citep{gou2021knowledge, wang2021knowledge, zagoruyko2016paying}.  More recently, general purpose models such as GPT-3.5 have been used to teach smaller models to perform question-answering tasks~\citep{zhang7llama}, assessment of student answers~\citep{li2023distilling}, follow specific types of instructions~\citep{tang2023domain}, and to improve output from existing smaller chatbots~\citep{chen2023phoenix}.

An important point in knowledge distillation is that there is almost always a trade made in exchange for the reducing model size.~\citet{gudibande2023false} make the point that small models attempting to replicate all capabilities of ChatGPT, for instance, are likely to face problems with generalization to prompts unlike those in the training samples.  They highlight how the benefit of knowledge distillation is focused on training small models to perform specific tasks -- one should not necessarily expect the small model to do all tasks well, but the small model can mimic the large one by specializing on a single task.  In this paper, we focus on the task of code summarization, and demonstrate how a small model can perform on par with the large one in this specialty.


